Accelerating the Development of Software-Defined Network Optimization Applications Using SOL

Software-defined networking (SDN) can enable diverse network management applications such as traffic engineering, service chaining, network function outsourcing, and topology reconfiguration. Realizing the benefits of SDN for these applications, however, entails addressing complex network optimizations that are central to these problems. Unfortunately, such optimization problems require significant manual effort and expertise to express and non-trivial computation and/or carefully crafted heuristics to solve. Our vision is to simplify the deployment of SDN applications using general high-level abstractions for capturing optimization requirements from which we can efficiently generate optimal solutions. To this end, we present SOL, a framework that demonstrates that it is indeed possible to simultaneously achieve generality and efficiency. The insight underlying SOL is that SDN applications can be recast within a unifying path-based optimization abstraction, from which it efficiently generates near-optimal solutions, and device configurations to implement those solutions. We illustrate the generality of SOL by prototyping diverse and new applications. We show that SOL simplifies the development of SDN-based network optimization applications and provides comparable or better scalability than custom optimization solutions.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\mypara{Path selection and optimality} While our empirical results
suggest that \pathPruneStrategyRandom or \pathPruneStrategyShortest
paths yield near-optimal solutions even with a small \pathPruneNmbr,
they also raise interesting theoretical questions: (1) Can we prove
that these selection strategies permit near-optimal solutions for
classes of problems?  (2) Can we provide hints to choose path
selection algorithms; e.g., is there some problem structure where one
strategy always works well?

\mypara{Expressiveness of \Name} Another question is understanding the spectrum
of applications that \Name can encompass. Our own experiences here have been
positive; we started from the NIDS/NIPS offloading application and were able to
apply the abstraction to a broader class of applications. That said, we do not
yet have a way to decide if a problem fits  the \Name paradigm and we plan to
address more applications to push this envelope further.

\mypara{Helping app developers use \Name} One direction of future work is to
run  user studies with SDN developers.  We are also looking forward to develop
tools/tutorials to help SDN application developers to use \Name.


==> extensions.tex <==
% -*- root: main.tex -*-
\section{Extensions}
\label{sec:extensions}

\Name users can benefit from  opt-in extensions
to  further reduce their development effort.  
Next, we present three such extensions that we currently support. We
plan to integrate other, concurrent ideas from the SDN literature as
future work (e.g.,~\cite{consistentupdate,onebigswitch}).


\mypara{Minimizing reconfiguration changes}
 In practice, network administrators may want to minimize the amount of
``churn'' induced by reconfiguration events.  Specifically, the network might
be in flux during reconfigurations and this may impact performance or induce
inconsistencies introduced by the reconfiguration.  
While other work focuses on  consistency properties (e.g., no loops or no
black-holes)~\cite{consistentupdate}, our intent here is more modest. We
want to  minimize the effective ``volume''  of reconfiguration required in
responding to network  dynamics (e.g., link failures or traffic matrix
changes).

To minimize the differences between configurations, we extend \Name
with new variables \totalDiff and $\epsilon_{\commodity,\Path}$ for
each $\commodity \in \commoditySet$ and $\Path \in
\pathSet{\commodity}$, and new constraints to model the distance
\totalDiff of the new configuration from the previous:\footnote{As
  expressed here, \totalDiff is the maximum
  $\epsilon_{\commodity,\Path}$ value, but it could also be defined as
  the sum of $\epsilon_{\commodity,\Path}$ values, for example.}
\begin{align*}
  & \forall \commodity\in\commoditySet, \forall\Path\in\pathSet{\commodity}: \\
  & \hspace{1em} \totalDiff \ge \epsilon_{\commodity, \Path} \ge 0;
  \hspace{1em} \flowFrac{\commodity}{\Path} + \epsilon_{\commodity, \Path} \geq 
  \prevFlowFrac{\commodity}{\Path} \geq \flowFrac{\commodity}{\Path} - \epsilon_{\commodity, \Path}
\end{align*}
Here, \prevFlowFrac{\commodity}{\Path} is a constant that denotes the
value of \flowFrac{\commodity}{\Path} resulting from the previous
optimization.  We can then extend the objective function to minimize a
weighted combination of the original objective and the \totalDiff
obtained with a given weight \DiffWeight, e.g.:
\begin{align*}
  & \labelDiffedMaxNodeLoad(\nodeResource,\DiffWeight):\\
  & \mbox{minimize~} \left[\left((1-\DiffWeight)
    \times \max_{\node \in \nodeSet}~ \nodeLoad{\node}{\nodeResource}\right)
    + \left(\DiffWeight \times \totalDiff\right)\right] 
\end{align*}
if the previous objective was $\labelMaxNodeLoad(\nodeResource)$.

\mypara{Reacting to faults} Our focus here is on the reaction logic
rather than the fault detection mechanism; we assume that the control
platform (e.g., {\tt OpenDayLight}) has some mechanisms to
report such events to \Name.  We provide a basic mechanism to react to
node or link failures as follows.

The high-level idea is that we build
a simple dependency graph between the set of paths we have chosen
during generation (\secref{sec:path}) and the specific links,
switches, and middlebox nodes that these paths traverse.
 Given this,  we implement the following two-step heuristic.  As
a first step, we simply re-run the optimization with the old set of
selected paths excluding the specific paths impacted by the
failures. If the objective value is significantly worse, then we fall
back to  running the selection step again (i.e.,
selecting \pathPruneNmbr paths from the already generated paths for
each traffic class, either \pathPruneStrategyRandom or
\pathPruneStrategyShortest) and rerun the optimization.  This two-step
heuristic works well in the common case because (i) the time to run
the optimization is typically lower than the time for selection, and
(ii) we can often find  near-optimal solutions even with fewer paths
per traffic class.

Note that we can also naturally compose  this fault tolerance step with the
above $\labelDiffedMaxNodeLoad$  objective to ensure that the reconfiguration
does not induce too many changes in reacting to a failure. 
